About latent roles in forecasting players in team sports

Forecasting players in sports has grown in popularity due to the potential for a tactical advantage and the applicability of such research to multi-agent interaction systems. Team sports contain a significant social component that influences interactions between teammates and opponents. However, it still needs to be fully exploited. In this work, we hypothesize that each participant has a specific function in each action and that role-based interaction is critical for predicting players' future moves. We create RolFor, a novel end-to-end model for Role-based Forecasting. RolFor uses a new module we developed called Ordering Neural Networks (OrderNN) to permute the order of the players such that each player is assigned to a latent role. The latent role is then modeled with a RoleGCN. Thanks to its graph representation, it provides a fully learnable adjacency matrix that captures the relationships between roles and is subsequently used to forecast the players' future trajectories. Extensive experiments on a challenging NBA basketball dataset back up the importance of roles and justify our goal of modeling them using optimizable models. When an oracle provides roles, the proposed RolFor compares favorably to the current state-of-the-art (it ranks first in terms of ADE and second in terms of FDE errors). However, training the end-to-end RolFor incurs the issues of differentiability of permutation methods, which we experimentally review. Finally, this work restates differentiable ranking as a difficult open problem and its great potential in conjunction with graph-based interaction models. Project is available at: https://www.pinlab.org/aboutlatentroles

==> src/backup/0.abstract_22_01.tex <==

\begin{abstract}
Forecasting players in sports has been gaining growing interest due to the potential for a tactical advantage and because the research is relevant to multi-agent interaction systems. Team sports share a complex social component that impacts the interactions between teammates and opponents, which has not been fully understood yet.
In this study, we speculate that each player has a particular role in every action and that role-based interaction is key to forecasting the future moves of players. We devise a new end-to-end model for Role-based Forecasting, which we dub \emph{RolFor}. RolFor adopts a new module we created called Ordering Neural Networks (OrderNN) to permute the players' order so each player is matched to a latent role. The latent role is then modeled with a so-called RoleGCN that, thanks to a graph representation, allows a fully learnable adjacency matrix that captures the relations among roles and is then used to predict the future trajectories of the players.
The claimed importance of roles is supported by thorough experiments on a challenging NBA basketball dataset.
When roles are provided by an oracle, the proposed RolFor is comparable to the current state-of-the-art (it ranks \#1 in terms of ADE, \#2 in terms of FDE errors).
However, the end-to-end RolFor is challenging to train, and we show experimentally that this is due to permutation algorithms not being fully differentiable. This highlights the need and the opportunity for fully-differentiable ranking methods in combination with graph-based interaction models.
\end{abstract}


==> src/backup/1.intro_07_02.tex <==
\section{Introduction}
% Generic Paragraph
Recent advances in visual recognition and sequence modeling have enabled novel objectives in athletic performance and sport analytics~\cite{rein2016big,merhej2021happened,morgulev2018sports}. One novel and challenging task is the multi-agent trajectory forecasting (See Fig. \ref{teaser}) of the players as a result of their observed current motion~\cite{evolvegraph, multimodalnba}. The difficulty is due to tactics, tight interaction of team players, the antagonist behavior of opponents, and the role assigned to each player in each action.
Traditional trajectory forecasting techniques~\cite{sociallstm, transformer, stgat, socialgan, socialstgcn} fall short in performance due to their general formulations and lack of sport-specific dynamics. Furthermore, trajectory forecasting methods must deal with the variable numbers of people in each scene (usually absent in games) and do not consider the presence of two opposing teams, the ball, or the finality in the given sport (e.g.~scoring). Most recent literature~~\cite{evolvegraph, multimodalnba} has started to address some of these objectives but, to our knowledge, none has modeled the role of players for specific actions. 
% See, for example, Fig.~\ref{teaser}, depicting the case of an NBA basketball play, where player A carries the ball into the basket area. Player C tries to delay its advance, and player B is A's teammate and waits for a pass.
% Our General Proposal 
We propose RoleFor, a novel graph-based encoder-decoder model that performs a robust prediction of the players' future trajectory, utilizing roles to comprehend their interactions. The players' positions and movements on the court often follow pre-defined schemes, so we assume that each player may be assigned a specific role. By proposing a role-based ordering of nodes in the graph, it is possible to establish a player order and learn specific role-specific relationships.

% \begin{center}
% \begin{figure}[!htp]
%     \centering
%     \includegraphics[scale=0.5]{src/figures/NBA_image.pdf}
     
%     \caption{The proposed RolFor forecasts the future positions of NBA basketball players, leveraging interaction patterns that are specific to their roles, e.g., \ be them the attacker A, the assist player B, or the marker C in the opponent team. First, RolFor identifies the latent role of players and orders them by an Ordering Neural Network module. Then it predicts future moves utilizing learned role-specific interaction patterns.
%     }\label{teaser}
    
% \end{figure}
% \end{center}

\begin{figure*}[!htp]
    \centering
        \includegraphics[scale =0.50]{src/figures/predictions.drawio.pdf}
    
    \caption{Example of multi-agent trajectory forecasting. We only plot one player for each team and the basketball for readability reasons.}
    \label{teaser}
\end{figure*}

To model relationships among team members, we are inspired by the related subject of human pose forecasting \FG{not sure that this is needed to state. Effectively you can remove this sentence and the paragraph is ok. Overall, our main statement is that one should consider latent roles, then use those as nodes in a GCN. Later in the paragraph one can say that we use the GCN method of sts-gcn, one of the best performers in pose forecasting.. mentioning the task adaptation seems a bit confusing, as the keypoints do not have anything to do with the latent roles, apart from being nodes}. 

The current best performers in-game forecasting~\cite{evolvegraph, socialstgcn} are based on graph convolutional networks (GCN)~\cite{kipfgcn}, but they do not consider roles. By contrast, in modern human pose forecasting techniques~\cite{stsgcn, sesgcn}, the nodes correspond to the (semantic) parts of the human body. Here we approximate body parts \FG{the word "approximate" raises lots of doubts on the relations of the two tasks. It's probably easier to just state that we model latent roles as nodes in the graph} with NBA players and their part-based interaction with an action-specific role-based interaction.
% Our Model
Our RoleFor model is composed of an ordering and a relational module. The former is an Ordering Network, which identifies latent roles and orders players according to them -- we use a well-known sorting approximation \cite{softrank} to order the latent projections of the players. In the latter, the game dynamics and trajectories are modeled using RoleGCN, where the nodes are the newly assigned roles, and the edges are their relations. As for recent GCNs models for Human Pose Forecasting, the adjacency matrix \cite{stsgcn} is learned \FG{here we may add a sentence stating that "learning this corresponds to learning the role-based player interaction", or something on those notes}. Our goal is to transition such concepts to learn role-role interactions \FG{avoid mentioning "transitions". It's maybe better to just state this as a modelling choice}.
% Roles exist
We assume roles exist, and many characteristics could dictate them -- e.g., marking the opponent, possessing the ball, and identifying the attacking and defending teams. However, we assume no prior knowledge
about roles.
Our goal is to learn latent roles with an end-to-end algorithm, only considering the future trajectory of all players.
To test our intuition about roles, we pre-processed the basketball dataset by assigning roles based on different methods (Table \ref{tab:oracle_orderings}) and using those in our RoleGCN. We produce SOTA results, confirming that finding good roles can improve the model performances.
Nevertheless, we found that current differentiable ordering methods face some limitations of backpropagation when inserted in complex models. 
In summary, our contributions are:
\begin{itemize}
    \item We observe that leveraging roles yields SoTA in trajectory forecasting.
    \item We propose an Order Neural Network module that creates a latent representation of the player's coordinates and orders them accordingly.
    \item We build a RoleGCN that learns the relations among roles.
    \item We observe that the current differentiable ordering approaches have some difficulties with backpropagation -- enabling little to no gradients to flow through -- when dealing with complex models.
\end{itemize}
\FG{I wouldn't use the word "we observe". One can state that "We demonstrate experimentally" (replacing each instance with this seems fine in both cases).}

==> src/backup/1.intro_22_01.tex <==
\section{Introduction}

% Generic Paragraph
Recent advances in visual recognition and sequence modeling have enabled novel objectives in athletic performance and sport analytics~\cite{rein2016big,merhej2021happened,morgulev2018sports}. One such novel task is the multi-agent trajectory forecasting of the players, as a result of their observed current motion~\cite{evolvegraph, multimodalnba}. This is a challenging goal, which is the result of tactics, the tight interaction of team players, the antagonist behavior of opponents, and the role assigned to each player in each action.

Traditional trajectory forecasting techniques~\cite{sociallstm, transformer, stgat, socialgan, socialstgcn} fall short in performance, due to their general formulations and lacking sport-specific dynamics. In fact, the trajectory forecasting methods need to deal with the changing numbers of people in the scene (normally not present in games), but they do not consider the presence of two opposing teams, the ball, nor the finality in the given sport (e.g.~scoring). Most recent literature~~\cite{evolvegraph, multimodalnba} has started to address some of these goals. However, to the best of our knowledge, none has modelled the role of players for the specific actions. See for example Fig.~\ref{teaser}, depicting the case of an NBA basketball play, where the player A carries the ball into the basket area, player C tries to delay its advance, player B is the team with A, waiting for its pass or to shoot.

% Our General Proposal 
Here we propose RoleFor, a novel graph-based encoder-decoder model that performs a robust prediction of the players' future trajectory, utilizing roles to learn about their interactions. The players' positions and movements on the court often follow pre-defined schemes, so we assume that each player may be assigned a specific role. By proposing a role-based ordering of nodes in the graph, it is possible to establish a player order and learn specific role-specific relationships.

\begin{center}
\begin{figure}[!htp]
    \centering
    \includegraphics[scale=0.5]{src/figures/NBA_image.pdf}
     
    \caption{The proposed RolFor forecasts the future positions of NBA basketball players, leveraging interaction patterns that are specific to their roles, e.g.\ be them the attacker A, the assist player B, or the marker C in the opponent team. First, RolFor identifies the latent role of players and orders them by an Ordering Neural Network module. Then it predicts future moves by means of learned role-specific interaction patterns.
    }\label{teaser}
    
\end{figure}
\end{center}
% Possible scenario in a basketball game where interactions between players dictate the future state of the game


% GCN
We are inspired by the related field of human pose forecasting, to model relations among team players. In fact, the current best performers in game forecasting~\cite{evolvegraph, socialstgcn} are based on graph convolutional networks (GCN)~\cite{kipfgcn}, but they do not consider roles. By contrast, in modern human pose forecasting techniques~\cite{stsgcn, sesgcn} the nodes correspond to the (semantic) parts of the human body, and the interaction between body parts is learned and encoded into the adjacency matrix of a GCN. Here we correspond body parts with NBA players and their part-based interaction with an action-specific role-based interaction.

% Our Model
The RoleFor model is composed of an ordering and a relational module. The first is achieved by an Ordering Network (Fig. \ref{ordernn}), which identifies latent roles and orders players according to them. We use a well-known sorting approximation \cite{softrank} to order the latent projections of the players. Secondly, the game dynamics and trajectories are modeled using RoleGCN, where the nodes are the newly assigned roles, and the edges are the relations. As for recent GCNs models for Human Pose Forecasting, the adjacency matrix \cite{stsgcn} is learned. Our goal is to transition such concepts to learn role-role interactions.

% Roles exist
Roles are not given explicitly in the dataset, although intuitively, roles exist, and many characteristics could dictate them, e.g., marking the opponent, possessing the ball, identifying the attacking team and the defending one. 
Since we are not given the ground truth, our goal is to learn latent roles with an end-to-end algorithm by only leveraging a final loss, optimizing the future trajectory of all players.
To test our intuition, we pre-processed the dataset by assigning roles based on different methods (Table \ref{tab:oracle_orderings}) and using those in our RoleGCN. We produce SOTA results, confirming that roles exist and the goal is to find the best one.
Nevertheless, we found that the current differentiable ordering methods have some limitations with the backpropagation inserted in complex models. 
In summary, our contributions are:
\begin{itemize}
    \item Observing that roles exist in sports and, if used, could produce SoTA results in trajectory forecasting.
    \item Creating an Order Neural Network module that creates a latent representation of the player's coordinates and orders them accordingly.
    \item Creating a RoleGCN that creates and learns the relations among roles.
    \item Finding out that the current differentiable ordering methods have some limitations with the backpropagation when dealing with complex models, allowing little to no gradients to pass through. 
\end{itemize}


==> src/backup/2.related_22_01.tex <==
\section{Related Work}
% In the following section, we first distinguish and discuss trajectory, game, and pose forecasting and then explain the differentiable algorithms we have used.

\paragraph{Trajectory Forecasting} 
The prediction of pedestrian movements has been studied to deal with realistic crowd simulation~\cite{pelechano07} or to improve vehicle collision avoidance~\cite{bhattacharyya2018long}; it was also used to improve the accuracy of tracking systems \cite{choi12, pellegrini10, yamaguchi11} and to study the intentions of individuals or groups of people \cite{lan12,xie18}.
Different models have been proposed to predict such trajectories, like deep learning models such as Long Short-Term Memory (LSTM) networks \cite{lstm}
with shared hidden states \cite{sociallstm}, multi-modal Generative Adversarial Networks (GANs) \cite{socialgan}, or inverse reinforcement learning \cite{activityfore}.
This group forecasting scenario finds its parallel in Game Forecasting, where it is necessary to model the movements of two opposing teams.

\paragraph{Game forecasting}
Associations such as National Basketball League or the English Premier League have used sophisticated tracking systems that allowed teams to gain insight into each game \cite{carling2008role}. Variational Autoencoders (VAEs) were used to model real-world basketball actions, showing that the offensive player trajectories are less predictable than the defense\cite{felsen2018will}. LSTM\cite{seidl10} were used to predict near-optimal defensive positions for soccer and basketball, respectively, as for predicting the player's movements during the game \cite{multimodalnba}. Variants of VAEs have also been used \cite{sun18} to generate trajectories for NBA players.
NBA player trajectory predictions were also studied in \cite{zhan18} and \cite{zheng17}, proposing a deep generative model based on VAE, LSTM, and RNN \cite{multimodalnba, lstm, rnn} and trained with weak supervision to predict trajectories for an entire team. Macro-intents for each player were inferred, where the players target a spot on the court they want to move to. 
Nonetheless, we did not encounter work estimating specific latent roles and learning the player interaction on those bases.

\paragraph{GCN-based forecasting}

Adopting a graph structure makes it possible to encode information and quantify shared information between nodes. SoA works in pose forecasting and learns specific terms for the specific joint-to-joint relation \cite{stsgcn, stgcn}.
Graphs are also widely used in trajectory forecasting and can be considered fully connected \cite{evolvegraph}, sparse or weighted. These structures distinctly model the interrelationships between nodes, and their combination can be a crucial factor. Also, Graph attention layers (GAT) are widely used in trajectory forecasting \cite{stgat, li2021grin} to learn the inter-player dependencies. 

Our idea is to use Graph Neural Networks with fully learnable adjacency matrices so that roles in a game (nodes) can freely communicate and help predict the future trajectories of the players.

\paragraph{Differentiable Ranking} 
Sorting and Ranking are two popular operations in information retrieval that, in our case, can be useful in identifying the role of players. 
When used in composition with other functions, sorting induces non-convexity, rendering model parameter optimization difficult.
On the other hand, the ranking operation outputs the positions, or ranks, of the input values in the sorted vector and, being a piece-wise constant function, the computation of gradients is way more complex, preventing gradient backpropagation.
Several recent works \cite{cuturi19, softrank} provide an approximation of the above operations to be used in a learnable framework.


==> src/backup/3.methodology_23_01.tex <==
\section{Methodology}
\LS{Iterated until this section}
This section formally defines the problem and illustrates our strategy to tackle it, focusing on the role assignment and encoding methods.
First, we will briefly explain how the Role-based Forecasting model (RoleFor) performs latent mapping, role assignment, and trajectory prediction.
Moreover, we will define the internal components, such as the Order Neural Network (OrderNN) that performs the ordering task, and then the RoleGCN that enables the learning process of the adjacency matrix that summarizes the relations among roles in a game. 

% Problem Formalization
\subsection{Problem Formalization}
We target to predict the future trajectory of all players, given the observed positions at past time frames. 

We denote the players by 2D vectors $x_{p, t}$ representing player $p$ at time $t$. The position of all players at time $t$ are aggregated into a matrix of 2D coordinates $X_t \in \mathbb{R}^{2 \times p}$. The motion history of all players is denoted by the tensor $X_{in} = [X_1, X_2, ..., X_T]$, which is constructed out of the matrices $X_t$  for frames $t = 1, ...,  T$. 
The goal is to predict the future $K$ players positions $X_{out} = [X_{T+1}, ..., X_{T+K}]$. 

% Role-based Forecasting model (RolFor)
\subsection{Role-based Forecasting model (RolFor)}
RoleFor uses two main components, the first one being the OrderNN (Section 3.2.1), which orders players according to their latent roles. We postulate the existence of latent roles learned in an end-to-end architecture to yield the best trajectory forecasting performance. From the OrderNN, we will consider $R$, the role vector, instead of $P$, the position vector. Notice that $R$ and $P$ have equal dimensions.

The graph is now defined as $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, where the nodes indicate the roles of each player and the edges capture the interaction among roles during the game. The graph $\mathcal{G}$ has $|\mathcal{V}| = T \times R$ nodes, which represent all $R$ roles across $T$ observed time frames. Edges in $\mathcal{E}$ are represented by a Spatio-Temporal adjacency matrix $A^{st} \in \mathbb{R}^{RT \times RT}$, relating the interactions of all roles at all times. Note that $A^{st}$ is learned, i.e., \ the model learns how players with different roles interact by learning how latent roles interact over time. 

% Order Neural Network
\subsubsection{Order Neural Network}
The Order Neural Network (Fig.~\ref{ordernn}) takes in input the initial coordinates $X_{in}$, maps them into a latent space and then, thanks to the use of a differentiable ranking method \cite{softrank}, it orders the latent vector into optimal roles $X_{role\_in}$, which has the same dimensionality of $X_{in}$. Note that roles get the corresponding position coordinates over subsequent time frames, so each role is now characterized by a spatio-temporal trajectory.

A simple example of a role assignment involves sorting players in ascending order based on their Euclidean distance from the ball.
This method is also used as a valuable proxy task, which we use for ablation studies (see Section \ref{4.experiments} Table \ref{tab:oracle_orderings}).
However, since RolFor is trained end-to-end, OrderNN is free to learn the ideal ordering that yields the best forecasting performance.

\par

\begin{center}
\begin{figure}[!htp]
    \centering
    \includegraphics[scale=1.1]{src/figures/OrderNN_module.drawio.pdf}
     
    \caption{Architecture of Order Neural Network}\label{ordernn}
    
\end{figure}
\end{center}

\paragraph{The differentiable ranking method} SoftRank, \cite{softrank} is a recent walkaround of the classic sorting and ranking algorithm. It is empirically shown that it achieves accurate approximation for both tasks. 
It is designed by constructing differentiable operators as projections onto the permutahedron, i.e., the convex hull of permutations, and using a reduction to isotonic optimization. 
The key takeaway of the method is to cast sorting and ranking operations as linear programs over the permutahedron. More precisely, it formulates the argsort and ranking operations as optimization problems over the set of permutations $\Sigma$. Then, to obtain continuous optimization problems, it introduces the permutahedron induced by
a vector $w \in \mathbb{R}^n$ as the convex hull of permutations of w:

\begin{equation}
        P(w) := conv(\left \{ w_\sigma:\sigma \in \Sigma \right \}) \subset \mathbb{R}^n
\end{equation}

SoftRank also relies on a regularization parameter $\varepsilon$, which is used to establish a trade-off between the loss function's differentiability and the optimum's accuracy. The greater the regularization factor ($\varepsilon  \rightarrow \infty$), the further the approximation will be from the permutation vertices, and the smoother the loss function gradient will be. On the opposite side, by picking an $\varepsilon \rightarrow 0$, the algorithm will produce results equal to the real permutation but with a lower degree of differentiability. 

After learning the ranking, we order the players according to it by employing a differentiable re-shuffling module.
The outputs of SoftRank are noted as $\left \{ s_i \right \}_{i=1}^{n}$ where \textit{n} is the number of rankings considered. At this point, we use a so-called \textit{base} matrix \textbf{B} with the number of rows and columns equal to the number of rankings. \textbf{B} will be used to store the real rankings $\left \{  p_i\right \}_{i=0}^n$. 

We then compute a $\left \{ \Delta_i \right \}_{i=1}^{n}$ matrix, which represents $\Delta_i = p_i-s_i$ for each position $\left \{  p_i\right \}_{i=0}^n$. The matrix $\Delta$ is used as the input as a rescaling function:

The re-shuffle process is a weighted combination. It is a real shuffling when the approximated rankings are integer and a differentiable shuffling instead when the ranking is fractional.
\begin{equation}
   M_i =  e^{(\frac{-\Delta}{scale})^2}
\end{equation}

\textbf{M} can be considered an array of weights for each position, with values closer to 1 being the predicted positions of each player. 
Finally, this will be used to recall the initial coordinates in an ordered manner:

\begin{equation}
    P_i=\left\{\begin{matrix}x_i' = \sum_{i = 1}^{n} M_i \cdot x_i
    \\ y_i' = \sum_{i = 1}^{n} M_i \cdot y_i\end{matrix}\right.
\end{equation}

% RoleGCN
\subsubsection{RoleGCN}
Once the latent roles are inferred, the graph $\mathcal{G}=(\mathcal{V}, \mathcal{E})$ represents each node $i \in \mathcal{V}$ as the player's role while the edges $(i, r) \in \mathcal{E}$ connect all the roles and describe their mutual interaction. 
RoleGCN (Fig~\ref{stsgcnorder}) will capture the underlying graph's relationships between different nodes on the court in the same time frame and the connection that one node has with itself over various time-frames, and let the adjacency matrices learn these interactions.

\begin{center}
\begin{figure}[!htp]
    \centering
    \includegraphics[scale =0.65]{src/figures/OrdeNN_architercture.drawio.pdf}
     
    \caption{Architecture of RoleFor that contains OrderNN and RoleGCN}\label{stsgcnorder}
    
\end{figure}
\end{center}

GCN \cite{kipfgcn} is a graph-based operation that works with nodes and edges. For nodes, it aims to learn an embedding containing information about the node itself and its neighborhood for each node in the graph. 
GCN generally takes pre-defined edges \cite{stgcn}, while in our case, edges express the relation between roles, so we let the model free to learn those parameters \cite{stsgcn}.
Thus, the learned adjacency matrices yield a quantitative description of the interplay among roles. 

The space-time cross-talk is realized by factoring the space-time adjacency matrix (as in \cite{stsgcn}) into the product of separate spatial and temporal adjacency matrices. $A^{st} = A^SA^t$

A separable space-time graph convolutional layer \textit{l} is written as follows:

\begin{equation}\label{STSlayer}
    H^{(l+1)} = \sigma(A^{s-(l)} A^{t-(l)} \mathcal{H}^{(l)}W^{(l)})
\end{equation}

It is similar to a classic GCN convolutional layer, where the equation is formulated as follows:

\begin{equation}\label{GCNlayer}
    H^{(l+1)} = \sigma(A^{st-(l)} \mathcal{H}^{(l)}W^{(l)})
\end{equation}

The critical difference is the factored $A^{s-(l)} A^{t-(l)}$ that allows better efficiency and allows full learnability. 

% Decoder
\subsubsection{Decoder}
First, we de-shuffle the permuted roles according to the inverse of $B$ to return to the original coordinates' position.
A Temporal convolution accomplishes the decoding and the prediction by applying multiple convolutional layers \cite{convauto} on the temporal dimension.
We adopt TCN for future frame prediction due to its performance and robustness.


==> src/backup/4.experiments_23_01.tex <==
\usepackage[tableposition=top]{caption}

\section{Experimental Evaluation}\label{4.experiments}
\LS{Iterated until this section}
In this section, we introduce the NBA benchmark dataset and metrics, then the trajectory forecasting results, and investigate why learning E2E roles is challenging, including a sorting module.

% Dataset
\subsection{Dataset}
For our experiments, we use NBA SportVU \cite{felsen2018will}. It contains player and ball trajectories for 631 games from the 2015-2016 NBA season. Similar to previous work \cite{sun18}, we focus on just two teams and consider all their games.
We rely on a dataset~ of $95,002$ 12-second sequences of the 2D basketball player and ball overhead-view point trajectories from $1247$ games in the $2015/16$ NBA season. Each sequence, sampled at $25$ Hz, has the same team on offense for the entire duration and ends in a shot, turnover, or foul.

\paragraph{Data Splits} As in \cite{felsen2018will}, the data is randomly split into train, validation, and test sets with $60'708$, $15'244$, and $19'050$ sequences respectively in each set.

% Trajectory Forecasting Metrics
\subsection{Trajectory Forecasting Metrics}
We adopt the metrics of ADE (Average Displacement Error) and FDE (Final Displacement Error), which are widely used in literature \cite{evolvegraph, multimodalnba}, for trajectory forecasting \cite{sociallstm, felsen2018will, socialgan}.
They are used to measure the error of the whole trajectory sequence and the final endpoints for each player.
Respectively:

\begin{equation}\label{ADE}
    ADE=\left \| \hat{T}_c-T_c \right \|_{2}^{2}
\end{equation}

\begin{equation}\label{FDE}
    FDE=\left \| \hat{E}_f-E_f \right \|_{2}^{2}
\end{equation}

Each observation has \textit{five} frames, which correspond to 2.0 seconds in a basketball scenario. The goal is to forecast the successive \textit{ten} frames (4.0 seconds).

In Eq.~\ref{ADE}, $\hat{T}_c$ represents the prediction for all future trajectories over the $c = 1, .., 10$ subsequent frames, and $T_c$ the ground truth. The same nomenclature is used in Eq.~\ref{FDE}, where $E$ is the matrix for the endpoints and $c = 1$ since we are only considering the last frame.


% Trajectory Forecasting Results
\subsection{Trajectory Forecasting Results}

\textit{So, do roles exist and does learning the role interaction yield state-of-the-art performance?} We answer this question by considering the easiest ordering: Euclidean distance of players from the ball.

In Table~\ref{tab:generic_results}, we report state-of-the-art techniques compared to the RolFor model, with the Euclidean distance ordering of players from the ball. In more detail, reported SoA techniques are:
\begin{itemize}
    \item EvolveGraph \cite{evolvegraph} proposes explicit relational structure recognition and prediction via latent interaction graphs among multiple interactive agents, the players. The model provides a multi-modal prediction hypothesis so that multiple outcomes are produced.
    It addresses the necessity of dynamic relational reasoning and adaptively
    evolving the interaction graphs. 
    
    \item Social GAN \cite{socialgan} is also a multi-modal model incorporating the social aspects of the players as well.
	A recurrent sequence-to-sequence model observes motion histories and predicts future behavior using a generative model and
    a pooling mechanism to aggregate information across players.
    
    \item STGAT \cite{stgat} is based on a sequence-to-sequence architecture to predict the future trajectories of players. Besides the spatial interactions captured by the graph attention mechanism at each time step, it adopts an extra LSTM to encode the temporal correlations of interactions.
    
    \item Social-STGCNN \cite{socialstgcn} substitutes the need for aggregation by modeling the interactions as a graph. Similar to \cite{} needs a pre-defined graph, allowing the leaning procedure only on the given edges.
    
\end{itemize}

RolFor in Table~\ref{tab:generic_results} yields the SoA forecasting performance in terms of ADE, 5.55 meters, second best in terms of FDE, 9.99 meters. RolFor sorts players according to their Euclidean distance from the ball, arranging them into a sequence of attackers (players detaining the ball in the considered action), alternating with defenders (players not detaining the ball). In particular, each attacker is followed by its marker, for which RolFor considers the closest to it in terms of Euclidean distance. As for all other reported SoA algorithms, RolFor considers that the teams are known. Finally, ``Oracular Permutation'' means that RolFor uses distances at the last future step, i.e., \ step 10 in the future, while any other reported algorithm uses only the observed 5 frames. We will investigate this in the next section.

A small neural network is capable of learning the Euclidean distance, and softRank should be capable of sorting the players according to it. So replacing the hand-defined distance computation with a Neural Network should be at least as effective.

We expect that a model with a sorting unit that learns sorting E2E in relation to the final forecasting goal should be capable of doing better than this, assuming all modules were effectively differentiable.

\input{src/tables/comparison_existing.tex}

% Further Experiments on Euclidean Ordering
\subsubsection{Further Experiments on Euclidean Ordering} \label{sec:eucl-ord}
We delve deeper into the results of RolFor in Table~\ref{tab:generic_results} and analyze the importance of each hand-defined Euclidean distance term in Table~\ref{tab:oracle_orderings}.

\textit{No ordering Vs. Simple ordering.}
The first forecasting result in the table neglects the player ordering and learns interaction terms between players, arranged in random order. It yields 6.34/11.5 ADE/FDE meters errors.

\noindent
Simple ordering stands for arranging all players in a list, according to their distance from the ball, at the last (5th) observed frame. This uncomplicated ordering is only negligibly better than no order. We conclude that a GCN model may deal with players in random order well, and it only benefits from ordering if it is informative.

\textit{Distance from the ball and marking.}
Results in the third row of the Table~\ref{tab:oracle_orderings} add marking to the ball distance ordering. Each player in the attacker team is matched with one from the defender team according to Euclidean distance.

\noindent
Performance improves in ADE, from 6.31 to 6.16 meters, and slightly degrades in terms of FDE, from 11.1 to 11.28. Overall
All distances are computed at the last observed frame. Furthermore, all distances are plain Euclidean distances, which a simple Neural Network may replicate or improve with E2E learning.

\textit{Distance from the ball and marking at future frames.}
The last row of Table~\ref{tab:oracle_orderings} considers the furthest future frame position for all distance computations.

\noindent
Note that the model assumes no future information in terms of positions. Future information is only used to order players (attackers ordered according to the distance from the ball at the 10th future frame, defenders ordered according to their minimum distance from each attacker, denoting their marking).
This encourages us to replace the hand-defined ordering with an E2E trained module, which we do in the next section.

\input{src/tables/ordering.tex}

% E2E Model with latent roles
\subsection{End to end Model with latent roles}

In this section, we leverage the full RolFor model, E2E trained. Here the first module, OrderNN, sorts players into their roles in the action, then the RoleGCN module reasons on their role-based interaction. Sorting into roles has benefited forecasting in Sec.~\ref{sec:eucl-ord}. Here we assume that roles are latent variables, which the OrderNN estimates, E2E, based on the best forecasting performance.

In Table~\ref{tab:e2e} we compare the hand-defined baseline (ball and marking distance on the last observed frame, scoring 6.16/11.28) against E2E model variants.

In Table~\ref{tab:e2e}, \textit{E2E} is learning to order, to encode the role-role interaction, and to forecast based on the encoder. This model is performing poorly at 12.12./15.02 ADE/FDE. Is this because the OrderNN is incapable of ordering, or is it because the OrderNN is not fully differentiable? 

In Table~\ref{tab:e2e}, the \textit{EuclDistEst} variant attempts to answer part of this question. Here we have pre-trained a small Neural Network module to compute the Euclidean distance based on the player's performance. We use the pre-trained module to sort players according to the ball. If the Euclidean distance estimator model were perfect, performance would be 6.31/11.1 (ADE/FDE), cf.~Table \ref{tab:oracle_orderings}. \textit{EuclDistEst} yields however 7.50/12.58. We attribute this mismatch to the residual errors in the Euclidean distance estimation, which, as it seems, matters. 

More surprisingly, in Table~\ref{tab:e2e}, \textit{E2E-finetune} starts from the \textit{EuclDistEst} variant and it fine-tunes it, E2E. The error increases to 12.08/14.97, so the model neglects the initialization and reverts to the \textit{E2E} performance. We attribute the discrepancy between \textit{EuclDistEst} and \textit{E2E} to the challenges in the SoftRank differentiability, as we further analyze in the next section. 

\input{src/tables/final_tabe.tex}

% Analysis of the Order Neural Network
\subsubsection{Analysis of the Order Neural Network}

Here we focus on confirming our claims on the issues of differentiability of Softrank. We set to order the players according to their ascending distance from the ball, at a specific frame, given their 2D coordinates. This allows us to test the first RolFor module, OrderNN, in isolation, cf.\ref{tab:ordering_results}.

In Table~\ref{tab:ordering_results}, we compare \textit{OrderNN E2E} against \textit{OrderNN EuclDistEst}. The first E2E trains the order of players and re-shuffles them. The second supervises the network by tasking it to learn the Euclidean distance between the players and the ball and then sort the distances according to SoftRank. 

We measure the ordering accuracy $p_{\text{ord}}$ as the percentage of players the models place in the correct order. In other words, we reproduce the top-k classification experiment as \cite{cuturi19}. The authors propose a loss for top-k classification between a ground truth class $ord \in [n]$ and a vector of soft ranks $\hat{ord} \in \mathbb{R}^n$, which is higher if the predicted soft ranks correctly place y in the top-k elements. 

\input{src/tables/ordering_accuracy.tex}


Observe from Table~\ref{tab:ordering_results} that learning Euclidean distances from 2D positions is an easier task for a deep neural network since SoftRank yields 71\% at the \textit{top-10} ordering accuracy $p_{\text{ord}}$.
It is also interesting to notice that when changing the \textit{top-k} ordering accuracy into ${5, 3, 1}$ we get similar results to \cite{softrank}.

By contrast, learning the ordering E2E from the 2D coordinates yields surprisingly low performance. Note in the table that \textit{OrderNN E2E} achieves a \textit{top-10} ordering accuracy of only 1\%.

% Robustness of RolFor to ordering errors
\subsection{Robustness of RolFor to ordering errors}

How much does misordering impact forecasting? We measure ADE and FDE forecasting errors when randomly altering the order provided by our best performing oracle RolFor (5.55/9.99 ADE/FDE, Table \ref{tab:oracle_orderings}).
In more detail, we consider the swap of two players \textit{Light Swap}, which can occur if the distance between them is relatively small. A more significant error can also quickly occur, e.g., if one role is not identified correctly and a player is inserted in a node that does not correspond to its actual role, making the whole order slip. We name this \textit{Light Insert}. In Table~\ref{tab:swap_error}, we consider the two potential sources of errors by randomly simulating one or both.
You can observe that the results are coherent with what we said previously Table \ref{tab:e2e}, where the RolFor \textit{EuclDistEst} has a \textit{top-10} ordering accuracy of $71\%$ yielding 7.50/12.58 while a Light Swap/Insert give 6.55/12.10 in ADE/FDE and $80\%$ \textit{top-10} ordering accuracy. 
This last Table \ref{tab:swap_error} highlights the importance of roles and their impact on the final trajectory accuracy.


\input{src/tables/erorr_ordering.tex}

% \subsection{Qualitative Results}
% We provide sample predictions taken from four different games. For the sake of visualization, we only randomly picked two players for each team and the basketball (divided by team, \textit{Blue: home}, \textit{Green: away} and \textit{Yellow: basketball}). Each game shows the predicted trajectory (\textit{dotted line}) versus the ground truth (\textit{continuous line}). The actions of both scenes start from the right and finish to the left of the field.

% Image \ref{fig:game1} represents an accurate prediction for all agents involved in the scene, considering the difficulty of predicting the endpoint. 

% Instead, Image \ref{fig:game2} shows the limits of our model. Close movements of the agents considered in the scene are hard to predict for the model. 

% \begin{figure*}[!htp]
%     \centering
%         \includegraphics[scale =0.50]{src/figures/Vanilla_STS_GCN_best_game_vs_gt (1).png}
    
%     \caption{Best scenario predictions for 2 different games. Each game contains the prediction for one player on each team and the basketball.}
%     \label{fig:game1}
% \end{figure*}

% \begin{figure*}[!htp]
%     \centering
%         \includegraphics[scale =0.50]{src/figures/Vanilla_STS_GCN_best_game_vs_gt20 (1).png}
    
%     \caption{Worst scenario predictions for 2 different games. Each game contains the prediction for one player on each team and the basketball.}
%     \label{fig:game2}
% \end{figure*}











==> src/backup/5.conclusion_23_01.tex <==
\section{Conclusions}

Our goal was to exploit and show that roles and social relations in sports could be effectively used to improve the current SoA models in game forecasting.

We have shown that roles exist by trying different definitions for them. The next step was to encode the player's coordinates into a latent space and then use the encoding to find an optimal latent role ordering.
The model used to perform trajectory forecasting is called RolFor, and it considers the input nodes of a graph indicating roles in a game. This single-graph framework favors the relation between roles and time, allowing better learning of the fully-trainable adjacency matrices for role-role and time-time interactions. The adoption of CNNs and the graph structure of the input allows the requirement of parameters to be only a fraction of the ones used in Transformers, GANs, and VAEs. 

% The most complex task was to permute the found latent roles using OrderNN, the main component of RolFor. When supervised, the Order Neural Network module correctly predicted $71\%$ \textit{top-10} of the permuted coordinates to learn the Euclidean distance between the players and the ball and then sort the distances according to SoftRank.

% The accuracy increases to $92\%$ when considering only \textit{top-1} order accuracy. In other words, the differentiable ranking method finds it hard to order all ten players perfectly.
% This is also confirmed when training RolFor end-to-end: the \textit{top-10} order accuracy drops to $1\%$ that pours into the trajectory performance, increasing the error by $54.2\%$ in ADE and $33.4\%$ in FDE.

Our observations underline the significant opportunity for future work to develop fully differentiable ordering modules, which can be effectively inserted in larger models and trained E2E. Such models would allow us to learn an optimal ordering of the input nodes to exploit an optimal role assignment for the nodes and, in our belief, would also help generalize our same approach to other related problems.
%As for future work, we would also like to find a fully differentiable method that allows us to learn an optimal ordering of the input nodes to exploit an optimal role assignment for the nodes. 






==> src/elsevierGuide.tex <==
%! Author = sbbfti
%! Date = 10/06/2020

\section{The Elsevier article class}

\paragraph{Installation} If the document class \emph{elsarticle} is not available on your computer, you can download and install the system package \emph{texlive-publishers} (Linux) or install the \LaTeX\ package \emph{elsarticle} using the package manager of your \TeX\ installation, which is typically \TeX\ Live or Mik\TeX.

\paragraph{Usage} Once the package is properly installed, you can use the document class \emph{elsarticle} to create a manuscript. Please make sure that your manuscript follows the guidelines in the Guide for Authors of the relevant journal. It is not necessary to typeset your manuscript in exactly the same way as an article, unless you are submitting to a camera-ready copy (CRC) journal.

\paragraph{Functionality} The Elsevier article class is based on the standard article class and supports almost all of the functionality of that class. In addition, it features commands and options to format the
\begin{itemize}
\item document style
\item baselineskip
\item front matter
\item keywords and MSC codes
\item theorems, definitions and proofs
\item lables of enumerations
\item citation style and labeling.
\end{itemize}

\section{Front matter}

The author names and affiliations could be formatted in two ways:
\begin{enumerate}[(1)]
\item Group the authors per affiliation.
\item Use footnotes to indicate the affiliations.
\end{enumerate}
See the front matter of this document for examples. You are recommended to conform your choice to the journal you are submitting to.

\section{Bibliography styles}

There are various bibliography styles available. You can select the style of your choice in the preamble of this document. These styles are Elsevier styles based on standard styles like Harvard and Vancouver. Please use Bib\TeX\ to generate your bibliography and include DOIs whenever available.

Here are two sample references: \cite{Feynman1963118,Dirac1953888}.

==> src/sections/6.ablation.tex <==
\appendix
\section{Ablation studies}
We decided to carry out additional studies on the adjacency matrix of graph $\mathcal{G}$. The focus of such experiments was to explore whether a different configuration of the learnable parameters of such matrices would positively impact the accuracy or vice-versa. 
\ref{tab:ablaadj} represents all of the approaches that we tried:

\input{src/tables/ablation.tex}

\begin{enumerate}

  \item Non-learnable Adjacency matrices using all 1's as constant values.
  
  \item Non-learnable Adjacency matrices using all 1's as constant values on the main diagonals and 0's off-diagonal.
 
  \item Learnable Adjacency matrices, both tempo and spatial with Uniform Initialization.

  \item Learnable parameter $\alpha$ as the diagonal term of the Adjacency matrices, and 0's off-diagonal.

  \item Learnable parameter $\alpha$ as the diagonal term of the Adjacency matrices, and $1-\alpha$ off-diagonal.

  \item Learnable parameters $\alpha$ and $\beta$. $\alpha$ as the diagonal term of the Adjacency matrices, and $\beta$ off-diagonal.
  
  \item Learnable Adjacency matrices, both tempo and spatial with Normal Initialization.
  
  \item Learnable Adjacency matrices, both tempo and spatial with Uniform Initialization and an additional hidden layer.
\end{enumerate}

\ref{tab:ablaadj} clearly shows better results for models with a higher number of learnable parameters, being the \textit{Learnable adjacency matrices} approach the best. 
Methods \textbf{1, 2, 4, 5} gave us similar results, meaning that a constant or close to constant adjacency matrix is not a viable approach to improve the accuracy. 
Empirical evidence also shows that a different initialization does not impact the final results, as for a deeper network, that only increases the number of learnable parameters.

==> src/tables/ablation.tex <==
\usepackage{floatrow}
\floatsetup[table]{capposition=above}

%Fix the table 
\begin{table*}[!htbp]
\centering
\begin{tabular}{l|l|l|c}
  \textbf{Types of Adjacency Matrix}   & \textbf{ADE} & \textbf{FDE} & \textbf{Number of Parameters (K)} \\ \hline
Non-Learnable Adj. Mat. Type 1                              & 7,16         & 12,6         & 13,88               \\ 
Non-Learnable Adj. Mat. Type 2                              & 7,51         & 12,9         & 13,88               \\ 
Learnable Adj. Matrices                                     & 6,33         & 11,6         & 17,40               \\ 
Learnable Diagonal Adj. Mat. Type 1                         & 7,09         & 13,014       & 13,89               \\ 
Learnable Diagonal Adj. Mat. Type 2                         & 7,218        & 13,155       & 13,89               \\ 
Learnable Diagonal Adj. Mat. Type 3                         & 6,998        & 12,87        & 13,89               \\ 
Learnable Adj. Matrices (Normal Initialization)             & 6,37         & 11,576       & 17,41               \\ 
Learnable Adj. Matrices (deeper network)                    & 6,34         & 11,55        & 42,56               \\ 
\end{tabular}%
\caption{Results of Ablation study using different methods to train the Adjacency Matrices}
\label{tab:ablaadj}

\end{table*}






==> src/tables/declaration.tex <==
\section{Declaration of Competing Interest}
The authors declare that they have no known competing financial
interests or personal relationships that could have appeared to influence the work reported in this paper.

% \section{CRediT authorship contribution statement}
% \textbf{Luca Scofano:} Conceptualization, Investigation, Project administration, Methodology, Writing – original draft, Visualization. \textbf{Alessio Sampieri:} Data curation, Investigation, Methodology, Writing – original draft. \textbf{Giuseppe Re:} Data curation, Conceptualization, Formal analysis, Supervision, Writing-review.\textbf{Matteo Almanza:} Data curation, Conceptualization, Formal analysis, Writing – original draft, \textbf{Alessandro Panconesi:} Conceptualization, Writing-review, Supervision. \textbf{Fabio Galasso:} Conceptualization, Writing-review, Supervision.

==> src/tables/erorr_ordering.tex <==
\begin{table}[h!]
\centering
\caption{Analysis of simulated errors in ordering}

\begin{tabular}{l|cc}
{Model} & ADE & FDE   \\ \hline
Oracular Ordering & 5.55                     & 9.99  \\
Light Swap                            & 6.55                     & 12.10 \\
Light Insert                          & 6.55                     & 12.10   \\
Light Swap + Light Insert             & 6.59                     & 12.08 \\
Heavy Swap + Heavy Insert             & 6.71                     & 12.25 \\ 
\end{tabular}
\label{tab:swap_error}
\end{table}






==> src/tables/euclidean_distance.tex <==
\begin{table}[!ht]
    \centering
    \caption{Error between the predicted distances and the correct euclidean distance from the ball}
    
    \begin{tabular}{|l|l|l|}
    \hline
        Batch Size & lr & MSE \\ \hline
        8 & 1,00E-02 & 60 \\ \hline
        128 & 1,00E-02 & 0,7 \\ \hline
        256 & 1,00E-02 & 0,8 \\ \hline
        256 & 1,00E-03 & 0,24 \\ \hline
        128 & 1,00E-03 & 0,1 \\ \hline
        128 & 1,00E-04 & 3,87 \\ \hline
    \end{tabular}
    \label{euclidean_distance}
\end{table}

==> src/tables/sota_results.tex <==
\begin{table}[H]
\begin{center}
\caption{Results of all considered models based on MAD and FAD.}

\begin{tabular}{ccc}
                                     & ADE                          & FAD                          \\ \hline
STS-GCN {[}oracle{]} & 5,53                                  & 9,47                                 \\ \hline 
Vanilla STS-GCN &  \textbf{6,20} & \textbf{9,87} \\
EvolveGraph & \textbf{5,73} & \textbf{8,65} \\ 
Social STGCNN & 6,42                                  & 10,04                                 \\ 
STGAT & 7,06                                  & 12,54                                 \\ 
SGAN & 5,88                                  & 10,36                                 \\ 

\end{tabular}
\label{tab:SOTAresults}
\end{center}
\end{table}

==> src/tables/sts_results.tex <==

\begin{table}[H]
\begin{center}
\caption{Results of all STS-GCN's configurations based on MAD and FAD.}

\begin{tabular}{ccc}
 & ADE & FAD \\ \hline
STS-GCN {[}oracle{]} & 5,53 & 9,47 \\ \hline
STS-GCN + Order NN & 8,30 & 12,86 \\ 
Vanilla STS-GCN & \textbf{6,20} & \textbf{9,87} \\ 
STS-GCN (Predicted Edpoint) & 10,2 & 15,6             \\ 
\end{tabular}
\label{tab:stsgcn_results}
\end{center}
\end{table}
